MULTIGAIN 2.0: MDP controller synthesis for multiple mean-payoff, LTL and steady-state constraints

We present MULTIGAIN 2.0, a major extension to the controller synthesis tool MULTIGAIN, built on top of the probabilistic model checker PRISM. This new version extends MULTIGAIN's multi-objective capabilities, by allowing for the formal verification and synthesis of controllers for probabilistic systems with multi-dimensional long-run average reward structures, steady-state constraints, and linear temporal logic properties. Additionally, MULTIGAIN 2.0 can modify the underlying linear program to prevent unbounded-memory and other unintuitive solutions and visualizes Pareto curves, in the two- and three-dimensional cases, to facilitate trade-off analysis in multi-objective scenarios.

==> 0_macros.tex <==
\renewcommand{\circ}{\bigcirc}
\newcommand{\classname}[1]{\texttt{#1}}
\newcommand{\gridworld}{\mathtt{Gridworld}}

\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\toolname}{\textsc{MultiGain} 2.0}

\def\code#1{\texttt{#1}}
\lstset{ %
language=bash,                % choose the language of the code
basicstyle=\footnotesize,       % the size of the fonts that are used for the code
numbers=none,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=true,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}

\renewcommand{\thesubfigure}{Figure \arabic{subfigure}}

%Arxiv refs.
%\newtoggle{arxiv}
%\newcommand{\arxivref}[2]{\iftoggle{arxiv}{#1}{#2}}
%\togglefalse{arxiv}

%LTL
%\newcommand \Until{{\mathbf{U}\kern-.1em}}
%\newcommand{\X}{{\mathbin{\mathbf{X}}}}
%\newcommand{\F}{{\ensumathbinremath{\mathbf{F}}}}
%\newcommand{\G}{{{\mathbf{G}}}}
%\newcommand{\U}{{\mathbin{\mathbf{U}}}}
%\newcommand{\true}{{\mathbin{\mathbf{tt}}}}
%\newcommand{\false}{{\mathbin{\mathbf{ff}}}}


\newcommand{\X}{{\ensuremath{\mathbf{X}}}}
\newcommand{\F}{{\ensuremath{\mathbf{F}}}}
\newcommand{\G}{{\ensuremath{\mathbf{G}}}}
\newcommand{\U}{{\ensuremath{\mathbf{U}}}}
\newcommand{\true}{{\ensuremath{\mathbf{tt}}}}
\newcommand{\false}{{\ensuremath{\mathbf{ff}}}}

% Standard math
\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Integers}{\mathbb{Z}}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}
\DeclareMathOperator*{\argopt}{arg\, opt}

%\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
%\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{min}}\;}
\newcommand{\eqdef}{\vcentcolon=}
\newcommand{\defeq}{=\vcentcolon}

\newcommand{\Dist}{\mathsf{Dist}}
\newcommand{\supp}{\mathsf{Supp}}
\newcommand{\post}{\mathsf{Post}}
\newcommand{\diff}{\mathsf{diff}}
\newcommand{\lfp}{\mathsf{lfp}}

% Layouting
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\qee}{\hfill$\triangle$}


% SG stuff
\newcommand{\opt}{\mathsf{opt}}
\renewcommand{\Box}{\square}
\renewcommand{\circ}{\bigcirc}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\SG}{\GG}
\newcommand{\Gsigma}{\GG^{(\sigma,\cdot)}}
\newcommand{\Gtau}{\GG^{(\cdot,\tau)}}
\newcommand{\Gst}{\GG^{(\sigma,\tau)}}
%\newcommand{\randomRandomOutcome}{\mathcal{SG}_{Algo}}
\newcommand{\randomRandomOutcome}{\GG_\mathsf{Algo}}
\newcommand{\connectedSG}{\mathsf{\GG_{reach}}}


\newcommand{\states}{\mathsf{S}}
\newcommand{\minStates}{\states_{\circ}}
\newcommand{\maxStates}{\states_{\Box}}
\newcommand{\initstate}{s_{0}}
\newcommand{\minstate}{s_{min}}
\newcommand{\maxstate}{s_{max}}
\newcommand{\state}{s}
%\newcommand{\state}{\mathsf{s}}
\newcommand{\action}{a}
%\newcommand{\action}{\mathsf{a}}
\newcommand{\act}{\mathsf{A}}
\newcommand{\actions}{\act}
\newcommand{\Av}{\mathsf{Av}}
\newcommand{\trans}{\delta}
%\newcommand{\stateMac}{\mathsf{s}}
\newcommand{\stateMac}{s}


\newcommand{\sink}{\mathsf{z}}
\newcommand{\sinks}{\mathsf{Z}}
\newcommand{\target}{\mathsf{f}}
\newcommand{\targets}{\mathsf{F}}

\newcommand{\Bop}{\mathcal{B}}
\newcommand{\BopD}{\mathcal{B}^{\mathsf{D}}}
\newcommand{\unknown}{\states^?}
\newcommand{\para}[1]{\smallskip\noindent{\bf#1}}
\newcommand{\parait}[1]{\smallskip\noindent{\it#1}}

% Objectives
\newcommand{\straa}{\sigma}
\newcommand{\strab}{\tau}
\newcommand{\straas}{\Sigma}
\newcommand{\strabs}{\Tau}
\newcommand{\strategies}{\mathbb{S}}
%\newcommand{\path}{\rho}
\newcommand{\Paths}{\mathsf{Paths}}

\newcommand{\reach}{\lozenge}
\newcommand{\stay}{\square}
\newcommand{\probability}{\mathcal{P}}
\newcommand{\val}{\mathsf{V}}
\newcommand{\lb}{\mathsf{L}}
\newcommand{\ub}{\mathsf{U}}
\newcommand{\bound}{\mathsf{b}}

% SVI
\newcommand{\svireach}{\mathsf{reach}}
\newcommand{\svistay}{\mathsf{stay}}
\newcommand{\svimin}{\mathsf{min}}
\newcommand{\svimax}{\mathsf{max}}
\newcommand{\svidec}{\mathsf{d}}
\newcommand{\svidecMin}{\mathsf{d_{l}}}
\newcommand{\svidecMax}{\mathsf{d_{u}}}
\newcommand{\posAttractor}{\mathsf{A^{attr_{>0}}}}
\newcommand{\almostSureAttractor}{\mathsf{A^{attr_{=1}}}}
\newcommand{\glb}{\mathsf{l}}
\newcommand{\gub}{\mathsf{u}}
\newcommand{\mec}{\mathsf{Y}}
\newcommand{\approximation}{\mathsf{apprx}_s}
\newcommand{\fix}{\mathsf{fix}}


%Algorithms
\newcommand{\SI}{\textsc{SI}}
\newcommand{\LPSI}{\SI_\textsc{LP}}
\newcommand{\SISI}{\SI_\textsc{SI}}
\newcommand{\TLPSI}{\textsc{T}\LPSI}
\newcommand{\TSISI}{\textsc{T}\SISI}

\newcommand{\VI}{\textsc{VI}}
\newcommand{\OVI}{\textsc{OVI}}
\newcommand{\OVIG}{\textsc{OVI_G}}
\newcommand{\BVI}{\textsc{BVI}}
\newcommand{\BVIG}{\textsc{BVI_G}}
\newcommand{\BVID}{\textsc{BVI_D}}
\newcommand{\WP}{\textsc{WP}}
\newcommand{\PTVI}{\textsc{PTVI}}
\newcommand{\PTBVI}{\textsc{PTBVI}}

%Appendix: Model-sets
\newcommand{\realcs}{REAL}
\newcommand{\mimic}{MIMIC}
\newcommand{\many}{RANDOM}
\newcommand{\largecs}{LARGE}



% Deflating
\newcommand{\bestExit}{\mathsf{bexit}}
% == Tikz
\newcommand{\drawcirc}{\node[draw,circle,minimum size=.7cm, outer sep=1pt]}
\newcommand{\drawbox}{\node[draw,rectangle,minimum size=.7cm, outer sep=1pt]}
\newcommand{\drawdummy}{\node[minimum size=0,inner sep=0]}
\newcommand{\drawnum}{\node[minimum size=.4cm,inner sep=1pt]}






%\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\vecl}[1]{\vec{\mathit{#1}}}
\newcommand{\dist}{\mathit{Dist}}
\newcommand{\poly}{\mathit{poly}}
%\newcommand{\ub}{\textbf{U:\ }}
%\newcommand{\lb}{\textbf{L:\ }}


\newcommand{\inits}{\hat s}
%\newcommand{\act}[1]{\mathit{Act}(#1)}
\newcommand{\pat}{\rho}
\newcommand{\Pat}{\mathsf{Runs}}
\newcommand{\fpat}{w}
\newcommand{\mem}{\mathsf{M}}
\newcommand{\Cone}{\mathsf{Cone}}
\newcommand{\calF}{\mathcal{F}}
%\newcommand{\mec}{\mathsf{MEC}}

\newcommand{\pr}{\mathbb P}	
\renewcommand{\Pr}[3]{\pr^{#1}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\PrS}[3]{\pr^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\expected}{\mathbb E}
\newcommand{\Ex}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}
\newcommand{\ExS}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}

\newcommand{\reward}{{r}}
\newcommand{\ex}{\vecl{exp}}
\newcommand{\sat}{\vecl{sat}}
\newcommand{\satscalar}{\mathit{sat}}
\newcommand{\psat}{\vecl{pr}}%{\vec{p^{sat}}}
\newcommand{\psatscalar}{\mathit{pr}}%{\mathit{p^{sat}}}

\newcommand{\lrLim}[1]{\mathrm{lr}(#1)}  %\lr{rew}{run}
\newcommand{\lrSf}[1]{\mathrm{lr}_{\mathrm{sup}}(#1)}  %\lrS{rew}{run}
\newcommand{\lrIf}[1]{\mathrm{lr}_{\mathrm{inf}}(#1)}  %\lrI{rew}{run}
%\newcommand{\lrInf}{\mathrm{lr}^{\mathrm{inf}}}  %\lrI{rew}{run}

\newcommand{\lrs}{\mathfrak {LR}}
\newcommand{\sss}{\mathcal S}
\newcommand{\rs}{R}
\newcommand{\ps}{\theta}
\newcommand{\mdp}{\mathcal G}
\newcommand{\mc}{\mathcal M}
\newcommand{\auto}{\mathcal{LDBA}(\varphi)}
\newcommand{\rmax}{R_{\max}}
\newcommand{\tran}[1]{\stackrel{#1}{\to}}
\newcommand{\accept}{\mathsf{acc}}
\newcommand{\amec}{\mathsf{AMEC}}
\newcommand{\acc}{\mathit{AccA}}
\newcommand{\lang}{\mathsf L}
\newcommand{\pair}[2]{\langle#1,#2\rangle}

%%%%%%%% Local and misc.:

\newcommand{\kda}{\mathbf{1}_a} %{\mathbbm{1}_a} %Kronecker's delta for a
%\newcommand{\reach}{\Diamond}%{\mathit{Reach}}
\newcommand{\stabi}[1]{\kappa_{#1}}
\newcommand{\lfa}{\mathit{lf}_a}
\newcommand{\vfreq}{\vecl{freq}}
\newcommand{\freq}{\mathrm{freq}}
\newcommand{\toss}{\mathit{toss}}
\newcommand{\leave}{\mathit{leave}}

% == TODOs



\newcommand{\fcirc}[1]{\tikz\draw[#1,fill=#1] (0,0) circle (.7ex);}

\newcommand{\rc}[1]{\textcolor{red}{#1}}
\definecolor{bblue}{rgb}{0,0,1}
\newcommand{\bc}[1]{\textcolor{bblue}{#1}}
%     \definecolor{ggreen}{rgb}{0,0.7,0.0}
\definecolor{ggreen}{rgb}{0,0.5,0.1}
\newcommand{\gc}[1]{\textcolor{ggreen}{#1}}
\definecolor{gb}{rgb}{0,0.8,1}
\newcommand{\black}[1]{\textcolor{black}{#1}}
\newcommand{\wc}[1]{\textcolor{white}{#1}}



==> 0_packages.tex <==
\usepackage[T1]{fontenc}
% T1 fonts will be used to generate the final print and online PDFs,
% so please use T1 fonts in your manuscript whenever possible.
% Other font encondings may result in incorrect characters.
%
\usepackage{graphicx}
% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following two lines
% to display URLs in blue roman font according to Springer's eBook style:
%\usepackage{color}
%\renewcommand\UrlFont{\color{blue}\rmfamily}
%
%\usepackage{amsthm}
\usepackage{times}
\usepackage{soul}
\usepackage{url}
\usepackage[utf8]{inputenc}
\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{bbding}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amssymb}
%\usepackage{bbm}
\usepackage[toc,page]{appendix}

\usepackage{tikz}
\usetikzlibrary{automata}

\usepackage{xspace}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{tabularx}
\usepackage{listings}
\usepackage{caption}
\usepackage{subcaption}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

%\usepackage{subfig}

